Quantum Computing and Visualization: A Disruptive Technological Change Ahead

The focus of this Visualization Viewpoints article is to provide some background on Quantum Computing (QC), to explore ideas related to how visualization helps in understanding QC, and examine how QC might be useful for visualization with the growth and maturation of both technologies in the future. In a quickly evolving technology landscape, QC is emerging as a promising pathway to overcome the growth limits in classical computing. In some cases, QC platforms offer the potential to vastly outperform the familiar classical computer by solving problems more quickly or that may be intractable on any known classical platform. As further performance gains for classical computing platforms are limited by diminishing Moore's Law scaling, QC platforms might be viewed as a potential successor to the current field of exascale-class platforms. While present-day QC hardware platforms are still limited in scale, the field of quantum computing is robust and rapidly advancing in terms of hardware capabilities, software environments for developing quantum algorithms, and educational programs for training the next generation of scientists and engineers. After a brief introduction to QC concepts, the focus of this article is to explore the interplay between the fields of visualization and QC. First, visualization has played a role in QC by providing the means to show representations of the quantum state of single-qubits in superposition states and multiple-qubits in entangled states. Second, there are a number of ways in which the field of visual data exploration and analysis may potentially benefit from this disruptive new technology though there are challenges going forward.

==> archive/xxx_notbeingused_01_introduction.tex <==

\input{fig_01}

\section{Introduction}

%
%Redesigning applications to be parallel required use of an explicit message passing protocol for implementing domain decomposition, synchronization, and gathering of partial results~\cite{Gropp2011}.
%
%
%In the present day, we find ourselves on the cusp of another such significant technology phase change: the dawn of quantum computing (\qx{}) and quantum information science and technology (\qist{})~\cite{Nielsen:Quantum:2010}.
%

The term \emph{classical computing} refers to a broad set of ideas and technologies from an era spanning the past five decades or more.
These technologies include the physical means for storing information, the mathematical basis for conceptually manipulating that information, and the semantic and syntactic way of expressing algorithms for implementing those manipulation concepts. 
Visualization as we commonly know it falls within this realm as well: it is the means for "seeing the unseeable", for transforming abstract information into readily comprehensible numbers~\cite{McCormick:1987}. The field of visualization has evolved within the rubric of classical computing constructs, ranging from  reformulating serial classical algorithms to perform better on parallel hardware to incorporating the principles of optics and radiation transport modeling to produce high-quality photorealistic images of models and data.

Similarly, the term \emph{quantum computing} (\qx{}) refers to a broad set of ideas and technologies related to the storage and manipulation of information.
However, the field of \qx{} %quantum Computing (\qx{}) 
%\qx{} is likely more than just another phase of computing technology evolution. 
is shaping up to be significantly more disruptive than previous changes we've been through with classical computing technology.
%The way we program and run codes on \qx{} platforms is radically different from practices and approaches for \emph{classical} computing systems of the past six or more decades~\cite{Nielsen:Quantum:2010}.
The language we use to describe concepts in \qx{}, terms like \emph{qubit}, \emph{quantum state}, \emph{superposition}, and \emph{entanglement} may be unfamiliar to many.
%
The information contained in classical and \qubits{} is completely different  thereby necessitating completely different visual data presentation metaphors as illustrated in Fig.~\ref{fig:summary:vis_classical_bits} and Fig.~\ref{fig:summary:vis_quantum_bits}.
%
The methods for programming these systems bear little resemblance to general purpose languages like C++ and Python as shown in Fig.~\ref{fig:summary:classical_program} and Fig.~\ref{fig:summary:quantum_circuit}.
%Many familiar computer organization concepts of von Neumann architectures like ALUs and memories~\cite{PattersonHennessy:2021} are not applicable in the \qx{} context. 
Unlike the practices we saw during the serial-vector-MPP evolution, there is no straightforward path for taking a serial classical code and transforming it somehow so that it will run on quantum platform.
Because \qx{} is so different than classical computing in so many respects,
 we expect the transition into \qx{} to be even more disruptive than any of the technological transitions we have seen so far. 
 This thought applies broadly to all of computing as well as specifically to the field of visualization.

%Because \qx{} platforms and approaches for creating quantum algorithms differ vastly from the \emph{classical} computing systems and approaches of the past six or more decades~\cite{Nielsen:Quantum:2010}, we expect that this new technology will be even more disruptive to the entire field of computing than the transitions to MPP or to accelerator-based platforms.
%, including scientific visual data analysis and exploration.
%
%As with previous disruptive technology changes, the transition into \qx{} will require us to go "back to the drawing board" to completely rethink how we approach many aspects of graphics and visualization.
%


\begin{comment}
    

Some  technology changes through the years have produced broad benefit without the need for any explicit code modifications.
During the era of Dennard Scaling 
%~\cite{Dennard:74} 
when processor clocks would roughly double in speed every 18-24 months, virtually all programs realized some level of performance gain due to the increase clock rate.
%
Other types of technology changes have been more disruptive and profound. One such disruption occurred during the transition from vector to MPP/distributed-memory supercomputers. During that era, it was typical for code architects to "go back to the drawing board" and rethink algorithmic design to accommodate changes in the underlying architecture.
The result was an evolution of serial to parallel code design patterns with concurrency levels ranging from  $O(2^6) \dots O(2^{20})$ or more on modern heterogeneous architectures.

\end{comment}

While the transition to \qx{} will likely be a bumpy one, 
there are several aspects of \qx{} that offer potential gains for graphics and visualization in terms of scalability of methods and quality of results. 
%
Fig.~\ref{fig:summary:classical_vs_quantum_ray_tracing} illustrates a key difference between classical and quantum raytracing. In the classical implementation, a ray is tested against objects in the scene one after another.
In the quantum implementation, a ray is tested against all objects in the scene with a single quantum operation applied at once to the $2^n$ quantum states created from $n$ entangled \qubits{}. 
%using quantum  operations applied to all potential quantum states.
%the idea of how ray-object intersections are performed one after another in classical raytracing but may in the quantum world, a single ray may be tested against all objects at once by leveraging the parallelism inherent in the quantum state and a fundamental \qx{} algorithm for searching.
%evaluates one ray at a time, whereas in the quantum world, 
%all ray-object intersections for all rays may be evaluated at once due to the inherent scaling of quantum state possible when using multiple \qubits{}. 
%\fix{Wes note to self: double check and revise preceding stmt.}
% classical and quantum walks
Fig.~\ref{fig:summary:classical_vs_quantum_walk} shows how a classical random walk converges to a probability distribution that looks like a Gaussian. 
On the other hand, the quantum walk produces a distribution that more thoroughly covers the mathematical space~\cite{Kempe:2003}  resulting in a potentially higher quality result for algorithms that use randomized methods based on walks. 
%One such example is distributed raytracing where a stochastic sampling using many rays at a pixel can capture "fuzzy phenomena" like depth of field, penumbras, and motion blur~\cite{Cook:84}.   
%For algorithms that use randomized sampling methods, taking more samples with a classical method converges to one part of the search space while taking more samples with quantum methods results in better distribution.
%In turn, the implication is that the quantum approach here may produce a better answer on the basis of better sampling. 

%There is significant opportunity for synergy between the fields of \qx{} and visualization, particularly when considering the ways that visualization may serve as a window into the "unseeable" quantum state. 
%Fig.~\ref{fig:summary:vis_classical_bits} shows "visualization" of the state of a set of classical bits, while Fig.~\ref{fig:summary:vis_quantum_bits} shows the visualization of the quantum state of three entangled \qubits{} each in a state of superposition. 

The objective for this article is to explore how visualization has helped understanding \qx{} concepts (\S\ref{sec:vis_for_quantum}) as well as to consider ways that visualization may benefit from \qx{} technology (\S\ref{sec:quantum_for_vis}).
%
Because \qx{} is so much different than classical computing, we first provide a brief introduction of key ideas and terminology (\S\ref{sec:qc_background}).

\input{fig_02}

\begin{comment}


% wes 1/19/2022, what follows through the end comment is the original sample introduction included with the template 

ifCLASSOPTIONcompsoc
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\else
\section{Introduction}
\label{sec:introduction}
\fi
% Computer Society journal (but not conference!) papers do something unusual
% with the very first section heading (almost always called "Introduction").
% They place it ABOVE the main text! IEEEtran.cls does not automatically do
% this for you, but you can achieve this effect with the provided
% \IEEEraisesectionheading{} command. Note the need to keep any \label that
% is to refer to the section immediately after \section in the above as
% \IEEEraisesectionheading puts \section within a raised box.


% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps (small caps for compsoc).
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
for IEEE Computer Society journal papers produced under \LaTeX\ using
IEEEtran.cls version 1.8b and later.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
I wish you the best of success.

\hfill mds
 
\hfill August 26, 2015

\subsection{Subsection Heading Here}
Subsection text here.

% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

\subsubsection{Subsubsection Heading Here}
Subsubsection text here.

\end{comment}

%\fix{Dan suggestions: For Fig 1, have 1a and 1b be one figure. Then create a new 2x2 figure using the existing 1c and 1d, talking about visualization of quantum state, and create two new figures that illustrate programs, e.g., one of them would be a boolean circuit of N bits and one would be a quantum circuit of log2 qubits.}






==> archive/xxx_notbeingused_03_qc_background.tex <==

\section{Quantum Computing Background}
\label{sec:qc_background}

% culled classical computing background text. it is in a "prerevisions" file

\vspace{4pt} % a wee bit of space improves readability

% true, but a bit off topic
%While \qx{} has been evolving as a field for several decades, it is only within the past few years that we have begun to see the emergence of readily accessible quantum platforms and methods for programming them.




\qx{} is fundamentally different from classical computing in terms of how the hardware built as well as how algorithms are designed and implemented.
%
\qx{} uses many terms that are not part of the classical computing landscape and may be unfamiliar,  
terms like \emph{qubit}, \emph{quantum state}, \emph{superposition}, and \emph{entanglement}.
%
The methods for programming these systems bear little resemblance to general purpose languages like C++ or Python.
%
%Many familiar classical computer organization concepts like ALUs and memories~\cite{PattersonHennessy:2021} are not applicable in the \qx{} context. 
Sidebar \S\ref{sec:sb:getting_started} provides a set of resources that are useful in learning more about \qx{}.
%

%From the perspective of the hardware, \qx{} platforms leverage completely different principles of physics than classical for representing information.
%
%From the perspective of software, the methods for programming \qx{} platforms are significantly different than those from the classical world due the the fundamental nature of the underlying physics of the hardware.
%

%\qx{} is much different than classical computing both in terms of the physics underlying the physical implementation of \qx{} platforms as well as the way we express algorithms that run on them.



In \qx{}, information is represented in the \emph{quantum state} on \emph{quantum bits}, or \qubits{}.
%
Unlike in the classical world where the state of a \emph{bit} is either a value of 0 or 1, the state of a \qubit{} is more complex owing to the nature of the  physics of quantum mechanics upon which it is constructed.
%
Intuitively, the \emph{quantum state} of a \qubit{} may be thought of as a probability rather than a discrete binary value. 

In the quantum world, we represent the \emph{quantum state} of a \qubit{} using \emph{Dirac} notation, which is the standard way of describing states in quantum mechanics.
In contrast to the classical bit states of either 0 or 1, a \qubit{} may be a combination of the states $\ket{0}$ and $\ket{1}$ at the same time.
These special states $\ket{0}$ and $\ket{1}$ are known as \emph{computational basis states}.
%and form an orthonormal basis for the vector space.
The quantum state $\ket{q}$ of a \qubit{} 
is a linear combination of these base states, where the combination of states is known as  a \emph{superposition} of base states~\cite{Nielsen:Quantum:2010}:
\begin{equation}
\ket{q} = \alpha\ket{0} + \beta\ket{1}
\label{eq:qubit-state}
\end{equation}
where $\alpha$ and $\beta$ are \emph{amplitudes} and
$\lbrace  \alpha,\beta \rbrace \in \mathbb{C}^2$.
%$\lbrace  \alpha,\beta \rbrace $ 
%
Born's rule states that  in a superposition of states, the modulus squared of the amplitude of a state is the probability of that state resulting after measurement. Furthermore, the sum of the squares of the amplitudes of all possible states in the superposition is equal to 1~\cite{Hidary:2019}.
Therefore, for the state $\ket{q}$ in Eq.~\ref{eq:qubit-state}, we have  ${|\alpha|}^2 + {|\beta|}^2 = 1$ and the probability of measuring state $\ket{0}$ state is ${|\alpha|}^2$ and state $\ket{1}$ is ${|\beta|}^2$.

\input{fig_03_pennies}

A useful analogy for a \emph{quantum state} is a coin toss.
%
While the coin is at rest and its state measured or observed, the coin is in either a heads or tails, $\ket{1}$ or $\ket{0}$ respectively as shown in the top and bottom rows of Fig.~\ref{fig:pennies}.
%
On the other hand, while the coin is spinning in the air, the coin is in a state of \emph{superposition} where its state is a combination of the heads and tails states as shown in the middle row of Fig.~\ref{fig:pennies}.
%
%It is not until you catch the coin and examine it that the state resolves into one of either heads or tails as shown in left half of Fig.~\ref{fig:pennies}.
In the quantum world, once the state of the \qubit{} is observed or measured, the value we observe is either 0 or 1. 
Upon measurement a \qubit{} its quantum state collapses and the $\alpha$ and $\beta$ are no longer accessible. 
%


% this image goes with the vis of single qubit section
\input{fig_04_single_qubit}



In addition to the idea of a probability of a heads or tails state, there is also the notion of \emph{quantum phase}. 
%
Consider the right column, middle row of Fig.~\ref{fig:pennies} where there are two possible configurations of a coin in a being-tossed state.
%
Both of these configurations appear to have the same probability of being a heads but they differ in \emph{phase} since one head points in a more westerly direction and the other points in a more easterly direction. 
%
While there are two different types of quantum phase, a \emph{global phase} and a \emph{relative phase}~\cite{Hidary:2019}, for the discussion here, the most important idea is that it is possible to have two (or more) quantum states that have identical probabilities for heads and tails state but that, like the right side of Fig.~\ref{fig:pennies}, are completely different states.

%then manipulated in \qx{} programs using a set of operators that conform to the principles of \emph{quantum mechanics} on devices capable of storing and manipulating quantum states using one of a number of different physical implementations. See Sidebar \S\ref{sec:sidebar_euler_angles} for more information about operations on quantum states..
%\fix{rewrite}



%Whereas the state of a classical \emph{bit} is either a value of 0 or 1, the state of a \qubit{} is more complicated owing to the nature of the  physics of quantum mechanics upon which it is constructed.
%


%\input{fig_secondary_image}

%\noindent\fix{Introduce the quantum state of a single qubit.}

Contemporary quantum platforms are not quite yet as usable as classical platforms due to the fact the underlying hardware is still maturing.
%
Unlike classical bits comprised of flip-flops that retain their state so long as voltage is present~\cite{PattersonHennessy:2021}, \qubits{} are able to reliably retain state for only a short amount of time, typically on the order of 100s of $\mu$seconds~\cite{IBM:Quantum:Cloud:2023}.
%
Present day systems are referred to as \emph{Noisy Intermediate Scale Quantum} (NISQ) platforms because the quantum state in \qubits{} and gates between them is subject to interference from external sources like heat and energetic particles in the environment~\cite{Preskill2018quantumcomputingin}.
%
As a result, to obtain reliable measurements from quantum programs, we must make repeated runs (1000s) of a given code to obtain a probability distribution of an answer.



%Due to the noise from thermal and external sources in \qubits{} and gates inherent in present day \emph{Noisy Intermediate Scale Quantum} (NISQ) platforms, we are required to make repeated measurements by rerunning the quantum program many times (1000s) to obtain answers having a high degree of confidence~\cite{Preskill2018quantumcomputingin}.
%\fix{RVB: mention that several/many quantum measurements are needed to obtain the distribution / numerical values of $\alpha$ and $\beta$. from Wes: a and b are not observable, right?}

Programming and the design of \qx{} algorithms is fundamentally different than the classical world. 
In the classical world, we read in data from disk then perform operations on it.
In the \qx{} world, most programs create an initial set of quantum states through a process of \emph{superposition} so that a \qubit{} is in a state that looks like Eq.~\ref{eq:qubit-state}, and then the quantum program performs operations on the quantum states, and then finally measures the \qubits{} to obtain the final answers.
The operations on quantum states must conform to a specific set of rules and constraints that may be thought of as applying a series of rotation matrices to the quantum state as further explained in Sidebar~\S\ref{sec:sidebar_euler_angles}.
%
Transferring classical data into quantum systems and then back out again is an area of ongoing research and engineering. 
There are several useful surveys of contemporary environments and approaches for creating and running quantum programs (c.f.~\cite{Hidary:2019}).

%In \qx{}, algorithm design and programming is all about specifying relationships between \qubits{} called \emph{entanglement} and then 
%manipulating the quantum states of single and multiple \qubits{} through specific operations that conform to a specific set of rules, namely the symmetries of quantum mechanics. 
%While we do introduce some of these concepts in the examples that follow, please
%refer to \S\ref{sec:sb:programming} for more information about \qx{} programming and programming environments, and refer to \S\ref{sec:sb:hardware}  for more information about current offerings of actual quantum hardware.  

%\fix{RVB: discussion of multiple qubits / quantum entanglement is missing!}
% right -- this comes later when we start talking about the visualization of multi-qubit systems

\begin{comment}


\fix{This text is from an earlier draft and will be redistributed}
%
If we simultaneously toss $n$ coins, we could describe the quantum state as that of an $n$-qubit system:
\begin{equation}
\ket{\psi} =\begin{bmatrix}
q_0 \\
q_1 \\
\vdots \\
q_{N-1} \\
\end{bmatrix}
\label{eq:quantum_state}
\end{equation}
where $N=2^n$, and each of the $q_i$ quantum states is as described in Eq.~\ref{eq:qubit-state}. 

Note that in the classical world, if we have $N$ bits then we have $N$ distinct states -- a linear relationship between the number of bits and the number of states.
In the quantum world, there is an exponential relationship between the number of \qubits{} and the number of states: if we have $N$ \qubits{}, then we have $2^N$ potential states.
%
Since the size of the quantum state space is exponential with the number of \qubits{}; this property  %is one of the characteristics that 
suggests the potential exists for \qx{} to solve certain types of problems that may be completely intractable in classical computing.

In addition to the concept of superposition of base states, another foundational idea in \qx{} is the idea  of \emph{entanglement}.
When two \qubits{} are entangled, 
%which refers to the fact that it is possible to create a relationship between the quantum states of two (or more) separate \qubits{}. 
%In other words, when \qubits{} are entangled,
the quantum state of one \qubit{} is correlated with the state of the other \qubit{}. 
The state of entanglement is created through the use of quantum programming methods (see \qx{} programming sidebar).

Whereas the quantum states of a single \qubit{} (Eq.~\ref{eq:qubit-state}) or of $n$ non-entangled \qubits{} are pure states, entangled \qubits{} result what is known as \emph{mixed states}. 
The mixed quantum state of an $n$-\qubit{} system is sometimes described with a \emph{density operator} or \emph{density matrix}, defined as $\rho$, where $\rho = \ket{\psi}\bra{\psi}$, which is the outer product of the state $\psi$ with itself: 
%Whereas on classical computers the state of each bit is independent of the states of all the other bits, things are different in the quantum world. Through quantum programming techniques, one may create states of entanglement between \qubits{}. When such an entanglement exists, the quantum state vector from Eq.~\ref{eq:quantum_state}, which reflects the state of $n$ independent or unentangled \qubits{}, is no longer sufficient to capture the complete state of the entangled system. 
%The \emph{density matrix}

\begin{equation}
\rho = \begin{bmatrix}
q_0 \\
q_1 \\
\vdots \\
q_{N-1} \\
\end{bmatrix} 
\begin{bmatrix}
q^*_0 q^*_1 \dots q^*_{N-1} 
\end{bmatrix} 
\end{equation}

\begin{equation}
\rho = \begin{bmatrix}
{|q_0|}^2 & q_0 q^*_0 & \dots & q_0 q^*_{N-1} \\
q_1 q*_0 & |q_1|^2 & \dots & q_1 q^*_{N-1} \\
\vdots & \vdots & \ddots & \vdots \\
q_{N-1} q^*_0 & q_{N-1} q^*_1  & \dots & |q_{N-1}|^2 \\
\end{bmatrix}
\label{eq:density_matrix}
\vspace{8pt}
\end{equation}


The process of expressing algorithms on quantum platforms involves specifying how entanglements are formed between \qubits{}. 
\fix{Briefly describe gate-based vs adiabatic platforms and point to hardware sidebar.}
\fix{Briefly mention programming environments for quantum platforms and point to software stack sidebar}. 




\subsection{Is Quantum Computing Better than Classical Computing?}

Given that \qubits{} are different than classical bits, what is so special about \qx{}? 
The answer lies in considering the number of unique states possible in classical bits versus \qubits{}.
With classical bits, the bit has two potential states: 0 or 1. 
With \qubits{}, the number of potential states is infinite for a single \qubit{}. 

What is Quantum Computing and why should you care? The objective here is to give a quick overview of QC technology, focusing mostly on the notion of \emph{quantum advantage}, the differences between a classical bit and a qubit, a quick overview of programming QC devices (quantum circuits), and a quick overview of hardware platforms and simulation environments.

qubits vs bits, superposition and entnaglement. 

The hope in 
Need to make clear where classical approaches are better and where we may see benefit from using quantum platforms.

The promise of quantum computers is that certain computational tasks might be executed exponentially faster on a quantum processor than on a classical processor~\cite{QuantumSupremacy:2019}. 

\subsection{Quantum Hardware Platforms}

Give a terse history of quantum hardware.


\subsection{Summary of Quantum Computing Accomplishments}

What has been done to date in QC? Give a quick overview of some of the foundational work in the QC space: Grover's, Shor's, Quantum Fourier Transform, Quantum Machine Learning, etc.


\end{comment}

==> archive/xxx_notbeingused__02_technology_vis.tex <==


\section{Timeline of Technology Changes Impacting Visualization}

\emph{Comment: we may decide to not develop and include this section. TBD.}

A brief history of technology evolution and its
impact on the field of graphics and visualization.
The objective here is to set the stage for the
fact that we as a community have been not just
coping with technology changes, but using them
to our advantage.

==> archive/xxx_notbeingused__03_qc_background_preRevisions.tex <==

\section{Quantum Computing Background}

\subsection{Classical Computing}

%For the purpose of this article, 
We use the term \emph{classical} computing to refer to a class of computational platforms and the means for expressing algorithms that run on those platforms.
Classical platforms are those that use a single binary digit to contain a single Boolean value that may be either True or False. 
In the present day, these classical \emph{bits} are stored in memories constructed from solid-state electronics (e.g, transistors) or in persistent storage using electromagnetic technologies (e.g., disk drives)~\cite{PattersonHennessy:2021}.
Over time during the past several decades, the density of bits per unit area of storage has roughly doubled every 18-24 months. This Moore's Law scaling will soon come to an end as the size of the "wires", or conducting channels in circuits, approaches one atom in width~\cite{national2019quantum}.

The way we program classical platforms reflects some fundamental underlying principles of physics of how bits are stored: when we write a value of True or False to a bit, that value persists until the next time we read it. Furthermore, we can perform repeated reads of a given bit of storage and the value of the bit doesn't change.
%
Modern programming languages like C++, Java, and so forth, present a programming model whereby we declare variables of varying types to which we assign values and perform computations using symbolic expressions using these variables. 
This form of programming language model has been in existence for many decades and is the backbone of most modern software.

The way we write code for doing visualization assumes we begin with a collection of data, often structured meshes or unstructured collections of values, and we transform these data into renderable primitives like line segments, surface triangles, or volumetric blocks. Then, we render those primitives into images using one of a different number of potential methods like surface-based or image-based methods. 

It is important to call out that in this classical approach to visualization, there is a readily accessible pathway from classical data through classical algorithms for visualization and rendering and finally into classical representation of results (pixels). 
Over the years, we have become accustomed to this pathway and have designed both hardware and software around its existence. 

%\fix{Add a paragraph about the classical approach to graphics, vis.}

\subsection{What is Quantum Computing?}

In brief, \qx{} is much different than classical computing both in terms of the physics underlying the physical implementation of \qx{} platforms as well as the way we express algorithms that run on them.
In \qx{}, information is encoded in a \emph{quantum state} on \emph{quantum bits}, or \qubits{}, then manipulated in \qx{} programs using a set of operators that conform to the principles of \emph{quantum mechanics} on devices capable of storing and manipulating quantum states using one of a number of different physical implementations. \fix{rewrite}


Whereas the state of a classical \emph{bit} is either a value of 0 or 1, the state of a \qubit{} is more complicated owing to the nature of the  physics of quantum mechanics upon which it is constructed.
%
As an  example, consider the process of a coin toss. While the coin is spinning in the air, the state of the coin is not fixed: it could be either heads or tails, each with a 50\% probability assuming a completely fair coin. It is not until you catch the coin and examine it that the state resolves into one of either heads or tails.

%\noindent\fix{Introduce the quantum state of a single qubit.}

In the quantum world, we represent the \emph{quantum state} of a \qubit{} using \emph{Dirac} notation, which is the standard way of describing states in quantum mechanics.
In contrast to the classical bit states of either 0 or 1, a \qubit{} may be in a combination of the states $\ket{0}$ and $\ket{1}$ at the same time.
These special states $\ket{0}$ and $\ket{1}$ are known as \emph{computational basis states} and form an orthonormal basis for the vector space.
The quantum state $\ket{q}$ of a \qubit{} 
is a linear combination of these base states, where the combination of states is known as  a \emph{superposition} of base states~\cite{Nielsen:Quantum:2010}:
\begin{equation}
\ket{q} = \alpha\ket{0} + \beta\ket{1}
\label{eq:qubit-state}
\end{equation}
where $\alpha$ and $\beta$ are \emph{probability amplitudes} of being in state $\ket{0}$ or $\ket{1}$, respectively. Here, $\alpha$ and $\beta$ encode the probability amplitudes as complex numbers. 
%Stated differently, the quantum state of a \qubit{} is a vector in a two-dimensional complex vector space. 
%The special states $\ket{0}$ and $\ket{1}$ are known as \emph{computational basis states} and form an orthonormal basis for this vector space.
The probabilities of a \qubit{} being in either state $\ket{0}$ or $\ket{1}$ are ${|\alpha|}^2$ and ${|\beta|}^2$.
The quantum state described in Eq.~\ref{eq:qubit-state} is referred to as a \emph{pure state} when ${|\alpha|}^2 + {|\beta|}^2 = 1$.

% wes removing this paragraph. it is a nice paragraph, but doesn't contribute much to the story. 
%In the classical world, we can examine a bit to determine whether it is in a 0 or 1 state. Somewhat counterintuitively, we cannot examine a \qubit{} to determine its full quantum state, namely the values of $\alpha$ and $\beta$. When we \emph{measure} a \qubit{}, we observe either a result of 0 with probability ${|\alpha|}^2$ or a result of 1 with probability ${|\beta|}^2$. This seeming paradox between the unobservable quantum state of a \qubit{} and the observations we make of its value are at the center of QC and QIST. 

Going back to the coin example, a classical bit is like the coin, it is either in heads or tails state.
In contrast, due to the nature of the superposition of base states, the \qubit{} may be in \emph{continuum} of states between $\ket{0}$ and $\ket{1}$. But, once the state of the \qubit{} is observed, known as \emph{quantum measurement}, the value we observe is either 0 or 1. The $\alpha$ and $\beta$ of the quantum state are no longer accessible once we observe the state of the \qubit{}.
Due to the noise inherent in \qubits{} and gates inherent in present day \emph{Noisy Intermediate Scale Quantum} (NISQ) platforms, we are required to make repeated measurements by rerunning the quantum program many times (1000s) to obtain answers having a high degree of confidence~\cite{Preskill2018quantumcomputingin}.
%\fix{RVB: mention that several/many quantum measurements are needed to obtain the distribution / numerical values of $\alpha$ and $\beta$. from Wes: a and b are not observable, right?}

Programming and the design of \qx{} algorithms is fundamentally different than the classical world. 
In the classical world, we read in data from disk then perform operations on it.
In the \qx{} world, most programs create an initial set of quantum states through a process of \emph{superposition} so that a \qubit{} is in a state that looks like Eq.~\ref{eq:qubit-state}, and then the quantum program performs operations on the quantum states, and then finally measures the \qubits{} to obtain the final answers.
Transferring classical data into quantum systems and then back out again is an area of ongoing research and engineering. 
There are several useful surveys of contemporary environments and approaches for creating and running quantum programs (c.f.~\cite{Hidary:2019}).
%In \qx{}, algorithm design and programming is all about specifying relationships between \qubits{} called \emph{entanglement} and then 
%manipulating the quantum states of single and multiple \qubits{} through specific operations that conform to a specific set of rules, namely the symmetries of quantum mechanics. 
%While we do introduce some of these concepts in the examples that follow, please
%refer to \S\ref{sec:sb:programming} for more information about \qx{} programming and programming environments, and refer to \S\ref{sec:sb:hardware}  for more information about current offerings of actual quantum hardware.  

%\fix{RVB: discussion of multiple qubits / quantum entanglement is missing!}
% right -- this comes later when we start talking about the visualization of multi-qubit systems

\begin{comment}


\fix{This text is from an earlier draft and will be redistributed}
%
If we simultaneously toss $n$ coins, we could describe the quantum state as that of an $n$-qubit system:
\begin{equation}
\ket{\psi} =\begin{bmatrix}
q_0 \\
q_1 \\
\vdots \\
q_{N-1} \\
\end{bmatrix}
\label{eq:quantum_state}
\end{equation}
where $N=2^n$, and each of the $q_i$ quantum states is as described in Eq.~\ref{eq:qubit-state}. 

Note that in the classical world, if we have $N$ bits then we have $N$ distinct states -- a linear relationship between the number of bits and the number of states.
In the quantum world, there is an exponential relationship between the number of \qubits{} and the number of states: if we have $N$ \qubits{}, then we have $2^N$ potential states.
%
Since the size of the quantum state space is exponential with the number of \qubits{}; this property  %is one of the characteristics that 
suggests the potential exists for \qx{} to solve certain types of problems that may be completely intractable in classical computing.

In addition to the concept of superposition of base states, another foundational idea in \qx{} is the idea  of \emph{entanglement}.
When two \qubits{} are entangled, 
%which refers to the fact that it is possible to create a relationship between the quantum states of two (or more) separate \qubits{}. 
%In other words, when \qubits{} are entangled,
the quantum state of one \qubit{} is correlated with the state of the other \qubit{}. 
The state of entanglement is created through the use of quantum programming methods (see \qx{} programming sidebar).

Whereas the quantum states of a single \qubit{} (Eq.~\ref{eq:qubit-state}) or of $n$ non-entangled \qubits{} are pure states, entangled \qubits{} result what is known as \emph{mixed states}. 
The mixed quantum state of an $n$-\qubit{} system is sometimes described with a \emph{density operator} or \emph{density matrix}, defined as $\rho$, where $\rho = \ket{\psi}\bra{\psi}$, which is the outer product of the state $\psi$ with itself: 
%Whereas on classical computers the state of each bit is independent of the states of all the other bits, things are different in the quantum world. Through quantum programming techniques, one may create states of entanglement between \qubits{}. When such an entanglement exists, the quantum state vector from Eq.~\ref{eq:quantum_state}, which reflects the state of $n$ independent or unentangled \qubits{}, is no longer sufficient to capture the complete state of the entangled system. 
%The \emph{density matrix}

\begin{equation}
\rho = \begin{bmatrix}
q_0 \\
q_1 \\
\vdots \\
q_{N-1} \\
\end{bmatrix} 
\begin{bmatrix}
q^*_0 q^*_1 \dots q^*_{N-1} 
\end{bmatrix} 
\end{equation}

\begin{equation}
\rho = \begin{bmatrix}
{|q_0|}^2 & q_0 q^*_0 & \dots & q_0 q^*_{N-1} \\
q_1 q*_0 & |q_1|^2 & \dots & q_1 q^*_{N-1} \\
\vdots & \vdots & \ddots & \vdots \\
q_{N-1} q^*_0 & q_{N-1} q^*_1  & \dots & |q_{N-1}|^2 \\
\end{bmatrix}
\label{eq:density_matrix}
\vspace{8pt}
\end{equation}


The process of expressing algorithms on quantum platforms involves specifying how entanglements are formed between \qubits{}. 
\fix{Briefly describe gate-based vs adiabatic platforms and point to hardware sidebar.}
\fix{Briefly mention programming environments for quantum platforms and point to software stack sidebar}. 




\subsection{Is Quantum Computing Better than Classical Computing?}

Given that \qubits{} are different than classical bits, what is so special about \qx{}? 
The answer lies in considering the number of unique states possible in classical bits versus \qubits{}.
With classical bits, the bit has two potential states: 0 or 1. 
With \qubits{}, the number of potential states is infinite for a single \qubit{}. 

What is Quantum Computing and why should you care? The objective here is to give a quick overview of QC technology, focusing mostly on the notion of \emph{quantum advantage}, the differences between a classical bit and a qubit, a quick overview of programming QC devices (quantum circuits), and a quick overview of hardware platforms and simulation environments.

qubits vs bits, superposition and entnaglement. 

The hope in 
Need to make clear where classical approaches are better and where we may see benefit from using quantum platforms.

The promise of quantum computers is that certain computational tasks might be executed exponentially faster on a quantum processor than on a classical processor~\cite{QuantumSupremacy:2019}. 

\subsection{Quantum Hardware Platforms}

Give a terse history of quantum hardware.


\subsection{Summary of Quantum Computing Accomplishments}

What has been done to date in QC? Give a quick overview of some of the foundational work in the QC space: Grover's, Shor's, Quantum Fourier Transform, Quantum Machine Learning, etc.


\end{comment}

==> biographies.tex <==

% wes 1/19/2022
% stuff in this file is included with the original template. ignoring it for now

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> fig_grovers_oracle.tex <==
\begin{figure*}[th!]
\centering
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/grovers_oracle_circuit.png}
         \caption{Circuit of 3 \qubits{} and the oracle for Grover's search.}
%         \caption{Two \qubit{} quantum circuit where each \qubit{} has been put into a state of equal superposition using a Hadamard gate. }
         \label{fig:3q_grovers_oracle_circuit}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/grovers_oracle_histogram.pdf}
         \caption{Histogram of probabilities.}
%         \caption{A histogram showing the probabilities of all possible $2^n$ quantum states of this $n=2$ \qubit{} system.}
         \label{fig:3q_grovers_oracle_histogram}
     \end{subfigure}
    \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/grovers_oracle_qsphere.pdf}
         \caption{Q-sphere}
%         \caption{A histogram showing the probabilities of all possible $2^n$ quantum states of this $n=2$ \qubit{} system.}
         \label{fig:3q_grovers_oracle_qsphere}
     \end{subfigure}
\caption{foo.} %\fix{Open question: whether or not to create a more complicated example for illustration rather than equal superposition}}
\label{fig:3q_grovers_oracle}
\end{figure*}


==> fig_secondary_image.tex <==
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/bitmap.png}
         \caption{Visualizing the state of 64 classical bits}
%         \caption{Two \qubit{} quantum circuit where each \qubit{} has been put into a state of equal superposition using a Hadamard gate. }
         \label{fig:summary:vis_classical_bits}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/3qubit_Hgates_qsphere_wide_v2.png}
         \caption{Visualizing the quantum state of 3 quantum bits (\qubits{}) in superposition.}
%         \caption{Two \qubit{} quantum circuit where each \qubit{} has been put into a state of equal superposition using a Hadamard gate. }
         \label{fig:summary:vis_quantum_bits}
     \end{subfigure} 
     %
       \begin{subfigure}[b]{0.50\textwidth}
         \centering
% insert image here         
\includegraphics[width=\textwidth]{images/PythonCode_conditional_flip_bits.png}
         \caption{Classical (python) code to flip bits 1 and 2 if bit 0 is set.}
         \label{fig:summary:classical_program}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
 % insert image here        
 \includegraphics[width=\textwidth]{images/QC_conditional_flip_bits.png}
         \caption{Quantum code (circuit) to flip the state of qubits 1 and 2 if the state of qubit 0 is $\ket{1}$}
%         \caption{Two \qubit{} quantum circuit where each \qubit{} has been put into a state of equal superposition using a Hadamard gate. }
         \label{fig:summary:vis_quantum_bits}
     \end{subfigure} 
     \vspace{8pt}
     \caption{comparing classical and quantum visualiation of state and program.}
     \label{fig:classical_vs_quantum}
     
\end{figure*}


==> sidebar_programming_QC_systems.tex <==
\section{Sidebar: Programming \qx{} Systems}
\label{sec:sb:programming}

 \fix{We don't have enough space for this sidebar.}

Explain the operations we used in the examples. 

Show the starting basis.

Then show the matrices for RX and RY gates. Explain these are performing rotations of the basis states. This idea should be immediately accessible to vis/graphics people. 

Give a quick overview of \qx{} gate-based programming environments.

Give a brief explanation of the difference between gate-based and adiabatic programming environments. 

Point to other references for more information.

Work in progress, expect a draft by Sunday evening.

==> sidebar_quantum_hardware.tex <==
\section{Sidebar: \qx{} Hardware}
\label{sec:sb:hardware}

 \fix{We don't have enough space for this sidebar.}
 
Give a quick survey of the state of \qx{} hardware systems. Will be very terse and point to other articles that provide summaries.

